Dynamically Tagged Groups of Metal-Poor Stars II. The Radial Velocity Experiment Data Release 6

Orbital characteristics based on Gaia Early Data Release 3 astrometric parameters are analyzed for ${\sim} 8,000$ metal-poor stars ([Fe/H] $\leq -0.8$) compiled from the RAdial Velocity Experiment (RAVE) Data Release 6. Selected as metal-poor candidates based on broadband photometry, RAVE collected moderate-resolution ($R \sim 7,500$) spectra in the region of the Ca triplet for these stars. About $20\%$ of the stars in this sample also have medium-resolution ($1,200 \lesssim R \lesssim 2,000$) validation spectra obtained over a four-year campaign from $2014$ to $2017$ with a variety of telescopes. We match the candidate stars to photometric metallicity determinations from the Huang et al. recalibration of the Sky Mapper Southern Survey Data Release 2. We obtain dynamical clusters of these stars from the orbital energy and cylindrical actions using the \HDBSCAN ~unsupervised learning algorithm. We identify $179$ Dynamically Tagged Groups (DTGs) with between $5$ and $35$ members; $67$ DTGs have at least $10$ member stars. Milky Way (MW) substructures such as Gaia-Sausage-Enceladus, the Metal-Weak Thick Disk, the Splashed Disk, Thamnos, the Helmi Stream, and LMS-1 (Wukong) are identified. Associations with MW globular clusters are determined for $10$ DTGs; no recognized MW dwarf galaxies were associated with any of our DTGs. Previously identified dynamical groups are also associated with our DTGs, with emphasis placed on their structural determination and possible new identifications. We identify chemically peculiar stars as members of several DTGs; we find $22$ DTGs that are associated with \textit{r}-process-enhanced stars. Carbon-enhanced metal-poor (CEMP) stars are identified among the targets with available spectroscopy, and we assign these to morphological groups following the approach given by Yoon et al.

==> Tables/cluster_orbital_table.tex <==
\startlongtable
\begin{deluxetable*}{l  r  c  c  r  r}
\tablecaption{Cluster Dynamical Parameters Determined by \AGAMA \label{tab:cluster_orbit}}
\tablehead{\colhead{Cluster} & \colhead{$N$ Stars} & \colhead{($\langle$v$_{\text{r}}\rangle$,$\langle$v$_{\phi}\rangle$,$\langle$v$_{\text{z}}\rangle$)} & \colhead{($\langle$J$_{\text{r}}\rangle$,$\langle$J$_{\phi}\rangle$,$\langle$J$_{\text{z}}\rangle$)} & \colhead{$\langle$E$\rangle$} & \colhead{$\langle$ecc$\rangle$}\\
\colhead{} & \colhead{} & \colhead{($\sigma_{\langle\text{v}_{\text{r}}\rangle}$,$\sigma_{\langle\text{v}_{\phi}\rangle}$,$\sigma_{\langle\text{v}_{\text{z}}\rangle}$)} & \colhead{($\sigma_{\langle\text{J}_{\text{r}}\rangle}$,$\sigma_{\langle\text{J}_{\phi}\rangle}$,$\sigma_{\langle\text{J}_{\text{z}}\rangle}$)} & \colhead{$\sigma_{\langle\text{E}\rangle}$} & \colhead{$\sigma_{\langle\text{ecc}\rangle}$}\\
\colhead{} & \colhead{} & \colhead{(km s$^{-1}$)} & \colhead{(kpc km s$^{-1}$)} & \colhead{(10$^{5}$ km$^{2}$ s$^{-2}$)} & \colhead{}}
\startdata
$DTG-1$ & $35$ & ($12.9$,$133.3$,$7.6$) & ($140.5$,$899.3$,$44.5$) & $-1.810$ & $0.419$ \\
 & & ($59.1$,$9.8$,$39.8$) & ($23.8$,$44.2$,$10.4$) & $0.018$ & $0.034$ \\
$DTG-2$ & $30$ & ($-8.7$,$259.0$,$0.7$) & ($23.8$,$2116.6$,$2.6$) & $-1.496$ & $0.126$ \\
 & & ($19.5$,$2.8$,$15.7$) & ($4.8$,$14.5$,$2.1$) & $0.003$ & $0.012$ \\
$DTG-3$ & $30$ & ($13.1$,$183.3$,$-3.7$) & ($46.7$,$1409.1$,$61.6$) & $-1.662$ & $0.210$ \\
 & & ($41.2$,$11.9$,$52.0$) & ($9.8$,$40.5$,$4.7$) & $0.012$ & $0.022$ \\
$DTG-4$ & $28$ & ($18.2$,$2.5$,$65.8$) & ($196.1$,$19.3$,$977.0$) & $-1.631$ & $0.475$ \\
 & & ($81.5$,$44.4$,$208.9$) & ($143.5$,$293.3$,$104.0$) & $0.053$ & $0.154$ \\
$DTG-5$ & $27$ & ($-2.5$,$189.7$,$-25.8$) & ($29.5$,$1392.6$,$105.7$) & $-1.655$ & $0.167$ \\
 & & ($35.7$,$16.0$,$67.3$) & ($11.4$,$53.0$,$6.0$) & $0.014$ & $0.035$ \\
$DTG-6$ & $24$ & ($-0.8$,$237.5$,$-1.6$) & ($3.4$,$1936.8$,$1.4$) & $-1.551$ & $0.050$ \\
 & & ($15.2$,$4.4$,$8.9$) & ($1.9$,$12.0$,$0.9$) & $0.004$ & $0.014$ \\
$DTG-7$ & $23$ & ($29.8$,$15.1$,$-2.3$) & ($573.1$,$107.5$,$31.5$) & $-1.845$ & $0.922$ \\
 & & ($75.8$,$16.6$,$36.6$) & ($28.8$,$121.9$,$7.3$) & $0.024$ & $0.044$ \\
$DTG-8$ & $23$ & ($1.2$,$2.8$,$3.6$) & ($826.9$,$24.6$,$38.5$) & $-1.708$ & $0.971$ \\
 & & ($144.0$,$9.5$,$30.3$) & ($32.8$,$78.7$,$21.0$) & $0.025$ & $0.033$ \\
$DTG-9$ & $23$ & ($13.2$,$204.9$,$0.0$) & ($21.3$,$1638.7$,$2.0$) & $-1.632$ & $0.134$ \\
 & & ($22.0$,$4.2$,$10.3$) & ($4.9$,$14.0$,$1.2$) & $0.003$ & $0.015$ \\
$DTG-10$ & $22$ & ($-5.4$,$187.5$,$3.5$) & ($45.2$,$1515.3$,$2.6$) & $-1.661$ & $0.199$ \\
 & & ($19.4$,$2.7$,$8.4$) & ($4.4$,$25.5$,$1.6$) & $0.009$ & $0.009$ \\
$DTG-11$ & $22$ & ($6.5$,$151.8$,$0.6$) & ($113.2$,$1094.1$,$28.6$) & $-1.759$ & $0.352$ \\
 & & ($50.7$,$7.1$,$32.7$) & ($12.0$,$28.0$,$8.6$) & $0.016$ & $0.017$ \\
$DTG-12$ & $21$ & ($21.2$,$5.3$,$-26.8$) & ($608.3$,$41.3$,$201.8$) & $-1.717$ & $0.902$ \\
 & & ($126.6$,$23.3$,$98.2$) & ($41.0$,$156.0$,$16.4$) & $0.020$ & $0.037$ \\
$DTG-13$ & $21$ & ($1.2$,$264.3$,$6.7$) & ($35.3$,$2146.5$,$2.3$) & $-1.485$ & $0.152$ \\
 & & ($24.5$,$4.5$,$9.1$) & ($3.6$,$8.6$,$1.1$) & $0.002$ & $0.008$ \\
$DTG-14$ & $20$ & ($24.2$,$113.7$,$-120.4$) & ($158.3$,$844.3$,$298.2$) & $-1.691$ & $0.430$ \\
 & & ($79.6$,$15.4$,$91.4$) & ($29.8$,$83.6$,$24.2$) & $0.022$ & $0.038$ \\
$DTG-15$ & $20$ & ($11.4$,$171.8$,$1.8$) & ($77.1$,$1363.3$,$4.0$) & $-1.697$ & $0.268$ \\
 & & ($26.1$,$5.3$,$14.4$) & ($10.1$,$29.0$,$1.8$) & $0.006$ & $0.018$ \\
$DTG-16$ & $20$ & ($9.4$,$193.2$,$1.3$) & ($22.0$,$1370.9$,$131.7$) & $-1.650$ & $0.153$ \\
 & & ($45.8$,$13.2$,$86.3$) & ($27.3$,$64.5$,$9.5$) & $0.012$ & $0.079$ \\
$DTG-17$ & $19$ & ($11.3$,$-4.4$,$-15.1$) & ($609.6$,$-35.5$,$73.5$) & $-1.807$ & $0.910$ \\
 & & ($97.0$,$14.1$,$53.2$) & ($22.4$,$104.9$,$10.2$) & $0.020$ & $0.052$ \\
$DTG-18$ & $19$ & ($10.4$,$-63.1$,$-27.1$) & ($397.2$,$-430.5$,$57.9$) & $-1.847$ & $0.724$ \\
 & & ($103.6$,$13.0$,$40.8$) & ($46.7$,$99.5$,$13.4$) & $0.037$ & $0.038$ \\
$DTG-19$ & $19$ & ($7.7$,$231.2$,$3.6$) & ($1.8$,$1865.1$,$1.6$) & $-1.572$ & $0.038$ \\
 & & ($12.0$,$4.0$,$5.3$) & ($2.3$,$6.3$,$0.7$) & $0.001$ & $0.022$ \\
\pagebreak
$DTG-20$ & $18$ & ($-8.2$,$46.2$,$5.9$) & ($413.6$,$304.2$,$146.0$) & $-1.808$ & $0.808$ \\
 & & ($102.2$,$8.8$,$66.1$) & ($21.6$,$79.3$,$16.8$) & $0.030$ & $0.042$ \\
$DTG-21$ & $18$ & ($-8.3$,$215.7$,$-3.8$) & ($11.7$,$1503.0$,$49.1$) & $-1.655$ & $0.104$ \\
 & & ($21.1$,$15.9$,$45.4$) & ($6.7$,$27.2$,$3.8$) & $0.009$ & $0.034$ \\
$DTG-22$ & $17$ & ($11.6$,$115.9$,$-39.5$) & ($246.6$,$886.2$,$115.9$) & $-1.709$ & $0.520$ \\
 & & ($98.2$,$17.5$,$69.1$) & ($25.3$,$40.7$,$7.7$) & $0.011$ & $0.028$ \\
$DTG-23$ & $17$ & ($4.6$,$245.0$,$0.1$) & ($5.4$,$1983.4$,$1.9$) & $-1.538$ & $0.062$ \\
 & & ($10.4$,$2.6$,$10.2$) & ($1.7$,$9.2$,$0.8$) & $0.002$ & $0.010$ \\
$DTG-24$ & $16$ & ($124.2$,$9.4$,$4.6$) & ($963.0$,$80.8$,$39.3$) & $-1.626$ & $0.940$ \\
 & & ($219.6$,$13.0$,$40.3$) & ($19.2$,$102.5$,$16.5$) & $0.025$ & $0.035$ \\
$DTG-25$ & $15$ & ($-16.6$,$99.9$,$13.2$) & ($270.5$,$732.8$,$43.4$) & $-1.796$ & $0.578$ \\
 & & ($59.9$,$10.7$,$40.2$) & ($26.8$,$87.3$,$4.3$) & $0.022$ & $0.038$ \\
$DTG-26$ & $15$ & ($38.7$,$68.9$,$-4.0$) & ($439.3$,$498.2$,$68.5$) & $-1.768$ & $0.731$ \\
 & & ($105.1$,$14.5$,$50.6$) & ($29.3$,$112.4$,$15.1$) & $0.022$ & $0.040$ \\
$DTG-27$ & $15$ & ($2.6$,$19.7$,$-28.3$) & ($508.3$,$136.5$,$96.5$) & $-1.839$ & $0.848$ \\
 & & ($80.3$,$12.9$,$61.7$) & ($24.7$,$87.7$,$5.9$) & $0.023$ & $0.063$ \\
$DTG-28$ & $15$ & ($-292.3$,$9.1$,$-0.4$) & ($1451.2$,$66.0$,$30.7$) & $-1.441$ & $0.975$ \\
 & & ($32.2$,$13.6$,$47.8$) & ($56.9$,$98.8$,$29.0$) & $0.019$ & $0.017$ \\
$DTG-29$ & $14$ & ($-24.2$,$105.4$,$-6.4$) & ($301.5$,$898.3$,$55.8$) & $-1.711$ & $0.560$ \\
 & & ($79.8$,$10.3$,$42.7$) & ($14.9$,$46.8$,$14.0$) & $0.010$ & $0.020$ \\
$DTG-30$ & $14$ & ($-118.2$,$-11.5$,$-23.6$) & ($804.0$,$-92.1$,$115.9$) & $-1.664$ & $0.949$ \\
 & & ($193.7$,$14.9$,$63.5$) & ($30.4$,$103.6$,$10.7$) & $0.012$ & $0.038$ \\
$DTG-31$ & $14$ & ($0.8$,$230.2$,$2.5$) & ($1.9$,$1892.5$,$0.3$) & $-1.565$ & $0.036$ \\
 & & ($13.3$,$2.1$,$6.6$) & ($2.0$,$10.3$,$0.1$) & $0.003$ & $0.020$ \\
$DTG-32$ & $14$ & ($62.7$,$161.6$,$69.6$) & ($115.5$,$1282.7$,$116.8$) & $-1.641$ & $0.331$ \\
 & & ($78.6$,$26.4$,$47.1$) & ($21.0$,$27.5$,$7.6$) & $0.007$ & $0.028$ \\
$DTG-33$ & $13$ & ($-26.9$,$166.1$,$64.2$) & ($34.0$,$828.0$,$129.8$) & $-1.856$ & $0.240$ \\
 & & ($5.6$,$3.6$,$11.1$) & ($9.0$,$41.8$,$7.5$) & $0.009$ & $0.036$ \\
$DTG-34$ & $13$ & ($-32.6$,$48.9$,$-103.9$) & ($242.7$,$232.7$,$534.5$) & $-1.788$ & $0.617$ \\
 & & ($85.2$,$47.7$,$200.8$) & ($100.1$,$201.9$,$47.9$) & $0.028$ & $0.162$ \\
$DTG-35$ & $13$ & ($35.2$,$205.4$,$-7.3$) & ($31.5$,$1520.2$,$36.7$) & $-1.648$ & $0.166$ \\
 & & ($55.4$,$7.8$,$43.6$) & ($9.7$,$16.8$,$3.1$) & $0.008$ & $0.026$ \\
$DTG-36$ & $13$ & ($-15.1$,$164.1$,$7.6$) & ($86.0$,$1284.1$,$40.8$) & $-1.696$ & $0.289$ \\
 & & ($34.7$,$7.7$,$45.8$) & ($7.2$,$34.1$,$3.8$) & $0.009$ & $0.014$ \\
$DTG-37$ & $12$ & ($-4.6$,$198.4$,$-5.8$) & ($17.6$,$1339.2$,$162.0$) & $-1.650$ & $0.133$ \\
 & & ($39.2$,$15.2$,$101.4$) & ($9.6$,$38.1$,$7.3$) & $0.011$ & $0.034$ \\
$DTG-38$ & $12$ & ($34.4$,$186.9$,$49.9$) & ($65.7$,$682.8$,$561.8$) & $-1.686$ & $0.297$ \\
 & & ($77.7$,$45.4$,$114.7$) & ($36.1$,$91.0$,$29.9$) & $0.032$ & $0.069$ \\
\pagebreak
$DTG-39$ & $12$ & ($-44.3$,$258.6$,$-0.8$) & ($53.0$,$2076.0$,$2.3$) & $-1.495$ & $0.188$ \\
 & & ($18.4$,$10.6$,$9.7$) & ($3.4$,$9.1$,$1.4$) & $0.002$ & $0.006$ \\
$DTG-40$ & $12$ & ($-1.9$,$188.5$,$1.9$) & ($39.2$,$1381.4$,$11.3$) & $-1.705$ & $0.194$ \\
 & & ($27.0$,$5.6$,$19.6$) & ($6.9$,$27.7$,$3.7$) & $0.006$ & $0.018$ \\
$DTG-41$ & $12$ & ($-111.3$,$224.1$,$3.8$) & ($175.7$,$1806.3$,$24.9$) & $-1.512$ & $0.351$ \\
 & & ($123.0$,$12.8$,$44.2$) & ($28.6$,$29.3$,$5.9$) & $0.012$ & $0.025$ \\
$DTG-42$ & $12$ & ($-18.9$,$149.1$,$-241.9$) & ($357.8$,$1132.5$,$1143.0$) & $-1.338$ & $0.435$ \\
 & & ($118.2$,$43.3$,$95.8$) & ($140.9$,$264.2$,$60.9$) & $0.056$ & $0.068$ \\
$DTG-43$ & $11$ & ($16.8$,$110.8$,$18.7$) & ($206.7$,$753.8$,$42.4$) & $-1.832$ & $0.515$ \\
 & & ($50.4$,$7.9$,$28.8$) & ($17.2$,$26.0$,$7.6$) & $0.008$ & $0.023$ \\
$DTG-44$ & $11$ & ($-116.4$,$46.7$,$-11.6$) & ($619.1$,$378.3$,$45.7$) & $-1.715$ & $0.814$ \\
 & & ($75.6$,$8.4$,$49.8$) & ($18.3$,$51.7$,$7.6$) & $0.011$ & $0.026$ \\
$DTG-45$ & $11$ & ($-38.7$,$1.2$,$24.8$) & ($570.2$,$3.7$,$129.3$) & $-1.798$ & $0.942$ \\
 & & ($128.2$,$12.8$,$66.6$) & ($21.8$,$77.8$,$7.8$) & $0.020$ & $0.044$ \\
$DTG-46$ & $11$ & ($13.1$,$-28.9$,$2.7$) & ($645.1$,$-213.8$,$119.7$) & $-1.717$ & $0.887$ \\
 & & ($165.7$,$7.1$,$48.9$) & ($30.3$,$55.8$,$11.3$) & $0.012$ & $0.026$ \\
$DTG-47$ & $11$ & ($-34.8$,$-119.0$,$12.9$) & ($197.6$,$-855.9$,$79.4$) & $-1.769$ & $0.481$ \\
 & & ($70.2$,$11.6$,$52.4$) & ($26.4$,$50.9$,$17.0$) & $0.025$ & $0.036$ \\
$DTG-48$ & $11$ & ($-12.5$,$225.4$,$13.9$) & ($3.3$,$1828.0$,$5.9$) & $-1.580$ & $0.050$ \\
 & & ($6.4$,$4.3$,$13.6$) & ($1.1$,$5.3$,$1.0$) & $0.002$ & $0.008$ \\
$DTG-49$ & $11$ & ($2.3$,$193.0$,$35.5$) & ($26.0$,$1225.6$,$60.1$) & $-1.738$ & $0.169$ \\
 & & ($37.3$,$8.1$,$54.1$) & ($6.4$,$27.6$,$5.9$) & $0.008$ & $0.021$ \\
$DTG-50$ & $11$ & ($-293.6$,$20.2$,$35.5$) & ($1660.4$,$185.1$,$40.2$) & $-1.354$ & $0.958$ \\
 & & ($15.7$,$16.0$,$41.2$) & ($42.5$,$140.7$,$17.3$) & $0.020$ & $0.028$ \\
$DTG-51$ & $11$ & ($99.4$,$158.2$,$9.0$) & ($192.1$,$1341.2$,$26.8$) & $-1.632$ & $0.407$ \\
 & & ($54.2$,$16.1$,$32.8$) & ($10.1$,$35.7$,$5.9$) & $0.008$ & $0.012$ \\
$DTG-52$ & $10$ & ($50.3$,$-96.2$,$-108.8$) & ($222.6$,$-638.9$,$247.7$) & $-1.756$ & $0.556$ \\
 & & ($87.8$,$26.7$,$65.9$) & ($44.3$,$85.0$,$18.7$) & $0.050$ & $0.018$ \\
$DTG-53$ & $10$ & ($52.3$,$152.8$,$-48.6$) & ($103.4$,$1175.5$,$238.5$) & $-1.632$ & $0.319$ \\
 & & ($37.3$,$27.8$,$98.7$) & ($15.4$,$30.6$,$10.6$) & $0.011$ & $0.022$ \\
$DTG-54$ & $10$ & ($7.9$,$206.7$,$-4.1$) & ($57.4$,$1759.2$,$142.2$) & $-1.522$ & $0.203$ \\
 & & ($65.3$,$22.1$,$83.7$) & ($19.1$,$53.3$,$5.7$) & $0.012$ & $0.035$ \\
$DTG-55$ & $10$ & ($38.9$,$115.8$,$-128.0$) & ($112.6$,$694.6$,$182.4$) & $-1.827$ & $0.416$ \\
 & & ($8.6$,$6.7$,$5.6$) & ($12.4$,$38.5$,$10.0$) & $0.008$ & $0.030$ \\
$DTG-56$ & $10$ & ($-28.2$,$-61.3$,$15.4$) & ($355.8$,$-399.2$,$156.7$) & $-1.802$ & $0.742$ \\
 & & ($65.1$,$12.7$,$94.9$) & ($31.6$,$78.7$,$12.4$) & $0.020$ & $0.052$ \\
$DTG-57$ & $10$ & ($17.6$,$-17.1$,$17.4$) & ($566.4$,$-113.0$,$321.9$) & $-1.702$ & $0.911$ \\
 & & ($157.9$,$8.5$,$130.4$) & ($58.5$,$60.8$,$18.8$) & $0.029$ & $0.038$ \\
\pagebreak
$DTG-58$ & $10$ & ($63.0$,$-4.2$,$27.0$) & ($575.2$,$-25.7$,$392.5$) & $-1.681$ & $0.930$ \\
 & & ($97.1$,$13.8$,$126.0$) & ($28.8$,$96.1$,$11.7$) & $0.018$ & $0.022$ \\
$DTG-59$ & $10$ & ($-4.0$,$274.1$,$4.6$) & ($56.2$,$2215.8$,$2.4$) & $-1.461$ & $0.188$ \\
 & & ($23.0$,$2.8$,$14.4$) & ($5.6$,$10.5$,$1.6$) & $0.002$ & $0.009$ \\
$DTG-60$ & $10$ & ($4.5$,$186.1$,$4.9$) & ($57.0$,$1505.3$,$14.5$) & $-1.651$ & $0.223$ \\
 & & ($41.1$,$7.2$,$29.4$) & ($4.1$,$7.3$,$2.2$) & $0.003$ & $0.008$ \\
$DTG-61$ & $10$ & ($5.5$,$238.7$,$-30.9$) & ($11.1$,$1957.6$,$18.0$) & $-1.533$ & $0.087$ \\
 & & ($23.4$,$10.4$,$25.7$) & ($7.2$,$9.6$,$2.0$) & $0.003$ & $0.030$ \\
$DTG-62$ & $10$ & ($1.6$,$183.5$,$13.2$) & ($57.1$,$1397.2$,$15.5$) & $-1.687$ & $0.231$ \\
 & & ($45.0$,$10.8$,$23.1$) & ($9.4$,$23.8$,$3.3$) & $0.003$ & $0.020$ \\
$DTG-63$ & $10$ & ($40.2$,$159.6$,$-12.9$) & ($136.1$,$1330.3$,$11.1$) & $-1.674$ & $0.352$ \\
 & & ($45.0$,$8.2$,$19.4$) & ($9.3$,$16.9$,$4.0$) & $0.005$ & $0.012$ \\
$DTG-64$ & $10$ & ($65.8$,$188.7$,$-39.2$) & ($73.7$,$1532.2$,$40.4$) & $-1.619$ & $0.252$ \\
 & & ($17.6$,$11.6$,$38.4$) & ($7.1$,$15.8$,$6.5$) & $0.005$ & $0.011$ \\
$DTG-65$ & $10$ & ($7.3$,$102.1$,$0.2$) & ($284.1$,$814.4$,$12.7$) & $-1.779$ & $0.571$ \\
 & & ($50.2$,$3.8$,$25.0$) & ($9.4$,$20.3$,$8.4$) & $0.012$ & $0.009$ \\
$DTG-66$ & $10$ & ($-328.0$,$22.4$,$40.4$) & ($1700.0$,$142.4$,$117.2$) & $-1.328$ & $0.971$ \\
 & & ($29.1$,$25.1$,$87.4$) & ($38.1$,$151.8$,$18.9$) & $0.026$ & $0.026$ \\
$DTG-67$ & $10$ & ($67.0$,$47.7$,$4.3$) & ($603.1$,$357.8$,$1988.7$) & $-1.271$ & $0.526$ \\
 & & ($142.4$,$45.3$,$295.9$) & ($208.9$,$308.1$,$76.7$) & $0.058$ & $0.079$ \\
$DTG-68$ & $9$ & ($-0.0$,$118.7$,$-3.2$) & ($164.7$,$804.2$,$87.0$) & $-1.801$ & $0.467$ \\
 & & ($50.1$,$7.1$,$75.3$) & ($8.3$,$41.0$,$6.8$) & $0.007$ & $0.029$ \\
$DTG-69$ & $9$ & ($1.7$,$66.3$,$23.3$) & ($409.8$,$478.8$,$43.9$) & $-1.807$ & $0.729$ \\
 & & ($83.8$,$10.4$,$43.2$) & ($33.9$,$77.8$,$6.3$) & $0.009$ & $0.035$ \\
$DTG-70$ & $9$ & ($-71.9$,$48.6$,$-1.7$) & ($533.5$,$379.0$,$22.2$) & $-1.776$ & $0.816$ \\
 & & ($56.1$,$8.4$,$36.2$) & ($17.0$,$53.0$,$5.3$) & $0.013$ & $0.025$ \\
$DTG-71$ & $9$ & ($9.6$,$1.3$,$-4.9$) & ($686.2$,$12.1$,$19.3$) & $-1.796$ & $0.945$ \\
 & & ($93.7$,$13.4$,$19.7$) & ($18.6$,$103.4$,$12.6$) & $0.015$ & $0.023$ \\
$DTG-72$ & $9$ & ($18.8$,$123.9$,$-12.9$) & ($127.4$,$662.2$,$107.5$) & $-1.879$ & $0.459$ \\
 & & ($59.0$,$15.6$,$49.9$) & ($21.8$,$44.5$,$6.7$) & $0.015$ & $0.033$ \\
$DTG-73$ & $9$ & ($33.2$,$121.9$,$-66.2$) & ($312.2$,$1011.8$,$114.4$) & $-1.636$ & $0.541$ \\
 & & ($121.5$,$12.1$,$28.6$) & ($21.6$,$58.6$,$12.1$) & $0.011$ & $0.021$ \\
$DTG-74$ & $9$ & ($-3.6$,$169.4$,$5.1$) & ($41.1$,$1169.3$,$270.6$) & $-1.651$ & $0.208$ \\
 & & ($59.8$,$17.8$,$129.4$) & ($18.2$,$49.7$,$8.4$) & $0.021$ & $0.045$ \\
$DTG-75$ & $9$ & ($211.3$,$2.4$,$-138.0$) & ($1255.6$,$39.2$,$285.5$) & $-1.424$ & $0.949$ \\
 & & ($109.9$,$23.2$,$85.0$) & ($44.5$,$151.8$,$24.3$) & $0.018$ & $0.019$ \\
$DTG-76$ & $9$ & ($180.8$,$-41.4$,$-11.1$) & ($848.6$,$-338.7$,$58.5$) & $-1.607$ & $0.856$ \\
 & & ($60.9$,$8.4$,$58.1$) & ($30.6$,$34.6$,$16.0$) & $0.015$ & $0.023$ \\
\pagebreak
$DTG-77$ & $9$ & ($14.2$,$137.6$,$14.3$) & ($99.0$,$707.0$,$260.5$) & $-1.792$ & $0.386$ \\
 & & ($78.3$,$16.1$,$80.2$) & ($21.8$,$40.5$,$15.1$) & $0.013$ & $0.045$ \\
$DTG-78$ & $9$ & ($43.1$,$-17.2$,$-132.1$) & ($472.8$,$-101.5$,$576.0$) & $-1.667$ & $0.771$ \\
 & & ($50.9$,$21.1$,$110.4$) & ($60.8$,$150.7$,$14.5$) & $0.031$ & $0.056$ \\
$DTG-79$ & $9$ & ($79.3$,$24.1$,$-33.9$) & ($476.6$,$148.3$,$247.5$) & $-1.776$ & $0.888$ \\
 & & ($85.0$,$15.0$,$115.6$) & ($40.1$,$93.6$,$13.1$) & $0.010$ & $0.057$ \\
$DTG-80$ & $9$ & ($211.7$,$4.0$,$18.0$) & ($1040.5$,$26.3$,$199.4$) & $-1.520$ & $0.958$ \\
 & & ($234.2$,$17.2$,$146.0$) & ($34.9$,$127.1$,$18.2$) & $0.013$ & $0.023$ \\
$DTG-81$ & $9$ & ($24.6$,$228.4$,$-0.4$) & ($18.8$,$1860.0$,$27.0$) & $-1.553$ & $0.119$ \\
 & & ($33.0$,$19.6$,$34.9$) & ($4.8$,$18.8$,$1.7$) & $0.005$ & $0.016$ \\
$DTG-82$ & $9$ & ($-15.5$,$189.5$,$4.3$) & ($41.2$,$1390.6$,$28.1$) & $-1.691$ & $0.199$ \\
 & & ($30.3$,$10.3$,$37.1$) & ($4.9$,$23.2$,$4.7$) & $0.004$ & $0.011$ \\
$DTG-83$ & $9$ & ($10.1$,$213.7$,$-5.3$) & ($11.6$,$1633.4$,$43.6$) & $-1.615$ & $0.098$ \\
 & & ($17.0$,$19.2$,$63.2$) & ($6.9$,$23.4$,$2.5$) & $0.005$ & $0.033$ \\
$DTG-84$ & $9$ & ($-0.9$,$205.0$,$-64.5$) & ($18.1$,$1643.2$,$55.9$) & $-1.603$ & $0.122$ \\
 & & ($31.7$,$10.3$,$12.7$) & ($4.9$,$35.2$,$2.6$) & $0.009$ & $0.018$ \\
$DTG-85$ & $9$ & ($39.8$,$168.1$,$-31.9$) & ($111.7$,$1319.7$,$34.0$) & $-1.673$ & $0.323$ \\
 & & ($58.6$,$9.4$,$39.7$) & ($11.0$,$11.9$,$4.1$) & $0.006$ & $0.015$ \\
$DTG-86$ & $9$ & ($-5.2$,$161.6$,$34.3$) & ($102.8$,$1247.7$,$92.8$) & $-1.675$ & $0.327$ \\
 & & ($65.9$,$15.8$,$40.6$) & ($14.2$,$24.6$,$5.2$) & $0.006$ & $0.028$ \\
$DTG-87$ & $9$ & ($-0.2$,$132.0$,$-3.3$) & ($180.1$,$1063.7$,$3.9$) & $-1.751$ & $0.434$ \\
 & & ($24.2$,$2.9$,$14.2$) & ($11.1$,$32.5$,$2.3$) & $0.008$ & $0.016$ \\
$DTG-88$ & $9$ & ($51.9$,$148.8$,$-0.8$) & ($269.0$,$1211.5$,$29.4$) & $-1.637$ & $0.485$ \\
 & & ($136.1$,$20.2$,$29.8$) & ($17.2$,$28.3$,$4.9$) & $0.005$ & $0.015$ \\
$DTG-89$ & $9$ & ($-8.4$,$201.5$,$6.8$) & ($11.1$,$1208.7$,$111.2$) & $-1.723$ & $0.112$ \\
 & & ($22.7$,$14.4$,$56.5$) & ($7.8$,$22.3$,$8.5$) & $0.004$ & $0.046$ \\
$DTG-90$ & $8$ & ($-20.9$,$116.9$,$-35.1$) & ($203.4$,$877.2$,$58.2$) & $-1.770$ & $0.487$ \\
 & & ($53.2$,$7.8$,$40.8$) & ($9.5$,$27.9$,$6.9$) & $0.009$ & $0.014$ \\
$DTG-91$ & $8$ & ($-23.4$,$165.6$,$-7.5$) & ($46.3$,$1007.2$,$107.2$) & $-1.786$ & $0.243$ \\
 & & ($32.5$,$9.6$,$64.0$) & ($18.3$,$42.8$,$3.6$) & $0.027$ & $0.041$ \\
$DTG-92$ & $8$ & ($325.5$,$-2.9$,$-31.5$) & ($1957.2$,$-21.7$,$52.1$) & $-1.286$ & $0.957$ \\
 & & ($25.6$,$21.1$,$88.0$) & ($47.3$,$165.1$,$14.2$) & $0.006$ & $0.014$ \\
$DTG-93$ & $8$ & ($11.8$,$94.2$,$9.3$) & ($244.6$,$696.9$,$129.7$) & $-1.772$ & $0.565$ \\
 & & ($35.0$,$4.8$,$66.2$) & ($14.2$,$34.3$,$4.4$) & $0.005$ & $0.022$ \\
$DTG-94$ & $8$ & ($48.1$,$118.3$,$7.2$) & ($147.0$,$874.4$,$213.1$) & $-1.719$ & $0.418$ \\
 & & ($61.4$,$21.7$,$100.6$) & ($16.6$,$41.2$,$5.6$) & $0.006$ & $0.026$ \\
$DTG-95$ & $8$ & ($114.7$,$-27.3$,$-17.4$) & ($741.6$,$-227.4$,$25.2$) & $-1.714$ & $0.910$ \\
 & & ($105.9$,$5.0$,$20.5$) & ($31.7$,$30.6$,$8.2$) & $0.012$ & $0.012$ \\
\pagebreak
$DTG-96$ & $8$ & ($-85.7$,$45.0$,$-17.6$) & ($674.6$,$370.4$,$82.4$) & $-1.669$ & $0.835$ \\
 & & ($144.9$,$13.1$,$63.7$) & ($10.8$,$46.0$,$11.8$) & $0.012$ & $0.031$ \\
$DTG-97$ & $8$ & ($-34.4$,$55.0$,$4.2$) & ($268.4$,$302.1$,$295.9$) & $-1.832$ & $0.714$ \\
 & & ($55.1$,$8.3$,$89.6$) & ($18.6$,$67.6$,$12.2$) & $0.040$ & $0.037$ \\
$DTG-98$ & $8$ & ($264.2$,$8.2$,$-2.5$) & ($1267.5$,$57.3$,$91.4$) & $-1.481$ & $0.957$ \\
 & & ($44.6$,$15.3$,$66.2$) & ($23.2$,$99.6$,$7.9$) & $0.008$ & $0.024$ \\
$DTG-99$ & $8$ & ($-6.5$,$68.5$,$-39.0$) & ($414.4$,$526.1$,$303.0$) & $-1.661$ & $0.679$ \\
 & & ($156.1$,$19.0$,$104.0$) & ($24.8$,$127.7$,$14.1$) & $0.029$ & $0.047$ \\
$DTG-100$ & $8$ & ($-148.0$,$81.6$,$19.1$) & ($691.1$,$686.7$,$155.2$) & $-1.544$ & $0.760$ \\
 & & ($88.4$,$22.6$,$90.5$) & ($31.4$,$71.4$,$18.6$) & $0.017$ & $0.020$ \\
$DTG-101$ & $8$ & ($-0.7$,$221.6$,$4.1$) & ($6.0$,$1813.2$,$1.0$) & $-1.587$ & $0.069$ \\
 & & ($14.7$,$3.9$,$7.1$) & ($2.1$,$11.5$,$0.6$) & $0.002$ & $0.010$ \\
$DTG-102$ & $8$ & ($20.5$,$-138.3$,$-2.8$) & ($94.5$,$-834.5$,$166.5$) & $-1.792$ & $0.359$ \\
 & & ($46.2$,$14.5$,$70.3$) & ($36.6$,$50.5$,$14.1$) & $0.015$ & $0.069$ \\
$DTG-103$ & $8$ & ($20.8$,$177.9$,$3.1$) & ($63.6$,$1465.5$,$4.1$) & $-1.667$ & $0.238$ \\
 & & ($13.3$,$3.4$,$18.8$) & ($6.9$,$10.9$,$1.2$) & $0.003$ & $0.012$ \\
$DTG-104$ & $8$ & ($27.6$,$185.8$,$39.7$) & ($42.3$,$1400.7$,$39.4$) & $-1.677$ & $0.200$ \\
 & & ($20.7$,$9.0$,$41.1$) & ($6.3$,$15.2$,$4.6$) & $0.004$ & $0.014$ \\
$DTG-105$ & $8$ & ($35.9$,$143.7$,$27.4$) & ($210.6$,$1152.9$,$45.9$) & $-1.675$ & $0.447$ \\
 & & ($106.8$,$11.3$,$43.7$) & ($9.0$,$26.8$,$4.4$) & $0.011$ & $0.013$ \\
$DTG-106$ & $7$ & ($40.1$,$115.1$,$-15.4$) & ($332.8$,$953.1$,$18.9$) & $-1.690$ & $0.570$ \\
 & & ($133.6$,$13.6$,$28.1$) & ($38.4$,$56.4$,$4.4$) & $0.009$ & $0.034$ \\
$DTG-107$ & $7$ & ($-2.8$,$182.5$,$107.4$) & ($106.8$,$1484.6$,$167.6$) & $-1.570$ & $0.293$ \\
 & & ($78.5$,$2.7$,$19.6$) & ($16.0$,$46.7$,$7.7$) & $0.015$ & $0.024$ \\
$DTG-108$ & $7$ & ($-17.5$,$75.8$,$44.1$) & ($326.2$,$569.3$,$112.0$) & $-1.783$ & $0.671$ \\
 & & ($65.0$,$6.7$,$56.1$) & ($8.1$,$41.5$,$6.3$) & $0.010$ & $0.008$ \\
$DTG-109$ & $7$ & ($-7.4$,$78.4$,$-20.0$) & ($356.2$,$580.7$,$165.9$) & $-1.732$ & $0.664$ \\
 & & ($97.3$,$11.0$,$63.6$) & ($11.4$,$50.6$,$8.1$) & $0.009$ & $0.019$ \\
$DTG-110$ & $7$ & ($-21.0$,$92.3$,$27.8$) & ($220.5$,$613.7$,$212.1$) & $-1.781$ & $0.562$ \\
 & & ($67.9$,$18.9$,$83.0$) & ($21.5$,$43.9$,$10.4$) & $0.009$ & $0.026$ \\
$DTG-111$ & $7$ & ($-28.2$,$-44.0$,$-77.3$) & ($488.5$,$-316.8$,$85.3$) & $-1.792$ & $0.800$ \\
 & & ($107.4$,$9.3$,$13.8$) & ($11.1$,$76.2$,$12.4$) & $0.023$ & $0.019$ \\
$DTG-112$ & $7$ & ($-114.4$,$50.5$,$-44.4$) & ($591.2$,$414.8$,$107.5$) & $-1.686$ & $0.811$ \\
 & & ($152.5$,$9.8$,$67.3$) & ($25.7$,$56.0$,$10.9$) & $0.006$ & $0.026$ \\
$DTG-113$ & $7$ & ($-53.6$,$1.8$,$-12.9$) & ($455.4$,$10.2$,$58.7$) & $-1.938$ & $0.854$ \\
 & & ($65.1$,$17.5$,$46.5$) & ($13.1$,$105.0$,$7.0$) & $0.002$ & $0.055$ \\
$DTG-114$ & $7$ & ($-34.2$,$54.6$,$-15.9$) & ($272.4$,$258.8$,$209.3$) & $-1.901$ & $0.747$ \\
 & & ($88.3$,$8.1$,$71.8$) & ($22.1$,$51.4$,$14.7$) & $0.011$ & $0.045$ \\
\pagebreak
$DTG-115$ & $7$ & ($-240.8$,$8.9$,$6.0$) & ($1124.3$,$81.9$,$100.5$) & $-1.533$ & $0.972$ \\
 & & ($324.3$,$12.8$,$68.5$) & ($27.0$,$105.9$,$19.7$) & $0.007$ & $0.023$ \\
$DTG-116$ & $7$ & ($-192.3$,$-21.1$,$54.8$) & ($831.5$,$-201.1$,$204.6$) & $-1.614$ & $0.907$ \\
 & & ($26.1$,$12.0$,$78.6$) & ($32.0$,$95.3$,$11.2$) & $0.015$ & $0.028$ \\
$DTG-117$ & $7$ & ($9.6$,$101.2$,$-57.2$) & ($120.0$,$439.8$,$336.9$) & $-1.844$ & $0.509$ \\
 & & ($50.6$,$32.0$,$119.6$) & ($43.4$,$115.6$,$7.2$) & $0.024$ & $0.104$ \\
$DTG-118$ & $7$ & ($6.8$,$244.0$,$-19.8$) & ($4.1$,$1943.3$,$4.9$) & $-1.547$ & $0.056$ \\
 & & ($6.0$,$3.7$,$12.3$) & ($1.4$,$2.5$,$0.8$) & $0.001$ & $0.010$ \\
$DTG-119$ & $7$ & ($-1.9$,$218.6$,$2.2$) & ($7.2$,$1743.0$,$3.3$) & $-1.606$ & $0.075$ \\
 & & ($16.7$,$5.0$,$13.9$) & ($1.6$,$6.3$,$0.4$) & $0.002$ & $0.009$ \\
$DTG-120$ & $7$ & ($45.3$,$191.3$,$-7.4$) & ($61.9$,$1569.6$,$5.1$) & $-1.634$ & $0.228$ \\
 & & ($30.6$,$8.7$,$12.0$) & ($4.7$,$12.3$,$1.4$) & $0.004$ & $0.008$ \\
$DTG-121$ & $7$ & ($45.6$,$183.9$,$0.5$) & ($73.5$,$1474.9$,$32.7$) & $-1.645$ & $0.255$ \\
 & & ($23.3$,$10.9$,$34.3$) & ($4.2$,$9.6$,$1.2$) & $0.004$ & $0.005$ \\
$DTG-122$ & $7$ & ($-42.3$,$188.3$,$-18.2$) & ($55.5$,$1470.5$,$52.3$) & $-1.642$ & $0.222$ \\
 & & ($38.4$,$23.1$,$39.8$) & ($5.1$,$13.4$,$3.9$) & $0.005$ & $0.010$ \\
$DTG-123$ & $7$ & ($-0.8$,$293.4$,$19.1$) & ($126.5$,$2352.5$,$4.7$) & $-1.405$ & $0.268$ \\
 & & ($40.3$,$1.2$,$17.4$) & ($10.1$,$22.2$,$2.4$) & $0.005$ & $0.011$ \\
$DTG-124$ & $7$ & ($69.5$,$138.3$,$19.0$) & ($179.6$,$1072.7$,$26.8$) & $-1.730$ & $0.432$ \\
 & & ($41.1$,$6.7$,$35.7$) & ($8.1$,$16.6$,$7.2$) & $0.005$ & $0.009$ \\
$DTG-125$ & $7$ & ($18.3$,$123.9$,$8.4$) & ($221.1$,$1035.2$,$14.3$) & $-1.729$ & $0.477$ \\
 & & ($46.2$,$8.1$,$25.3$) & ($8.9$,$25.2$,$2.8$) & $0.008$ & $0.011$ \\
$DTG-126$ & $7$ & ($-15.3$,$233.6$,$15.6$) & ($30.1$,$1642.6$,$80.9$) & $-1.586$ & $0.171$ \\
 & & ($35.7$,$21.6$,$52.6$) & ($5.7$,$32.8$,$5.7$) & $0.005$ & $0.034$ \\
$DTG-127$ & $7$ & ($45.3$,$-98.1$,$13.5$) & ($128.7$,$-423.9$,$202.8$) & $-1.914$ & $0.543$ \\
 & & ($68.1$,$17.4$,$59.2$) & ($40.7$,$73.6$,$14.1$) & $0.029$ & $0.060$ \\
$DTG-128$ & $7$ & ($-107.8$,$197.0$,$10.2$) & ($156.8$,$1588.5$,$6.3$) & $-1.585$ & $0.350$ \\
 & & ($8.9$,$4.7$,$15.0$) & ($4.9$,$39.0$,$3.1$) & $0.008$ & $0.009$ \\
$DTG-129$ & $7$ & ($-4.2$,$240.7$,$4.8$) & ($18.8$,$1947.0$,$82.5$) & $-1.512$ & $0.119$ \\
 & & ($22.8$,$11.8$,$66.4$) & ($9.3$,$37.4$,$7.7$) & $0.007$ & $0.034$ \\
$DTG-130$ & $6$ & ($44.9$,$182.5$,$-110.9$) & ($51.8$,$1343.9$,$186.2$) & $-1.623$ & $0.220$ \\
 & & ($15.5$,$27.2$,$24.4$) & ($13.5$,$19.2$,$4.2$) & $0.007$ & $0.028$ \\
$DTG-131$ & $6$ & ($22.3$,$185.4$,$-97.5$) & ($70.8$,$1450.6$,$128.5$) & $-1.608$ & $0.245$ \\
 & & ($62.4$,$13.1$,$7.8$) & ($14.8$,$9.1$,$8.1$) & $0.008$ & $0.025$ \\
$DTG-132$ & $6$ & ($82.9$,$136.4$,$74.7$) & ($157.0$,$950.1$,$167.1$) & $-1.710$ & $0.421$ \\
 & & ($83.7$,$11.2$,$33.0$) & ($11.9$,$37.2$,$2.2$) & $0.019$ & $0.013$ \\
$DTG-133$ & $6$ & ($-2.6$,$30.2$,$5.7$) & ($678.2$,$222.7$,$24.8$) & $-1.748$ & $0.904$ \\
 & & ($172.8$,$9.3$,$34.5$) & ($18.5$,$83.6$,$12.1$) & $0.015$ & $0.034$ \\
\pagebreak
$DTG-134$ & $6$ & ($-17.5$,$1.4$,$-70.1$) & ($432.1$,$12.3$,$185.5$) & $-1.880$ & $0.959$ \\
 & & ($63.9$,$8.1$,$94.5$) & ($11.7$,$46.5$,$4.2$) & $0.012$ & $0.022$ \\
$DTG-135$ & $6$ & ($-31.9$,$9.4$,$-1.2$) & ($468.9$,$59.2$,$150.0$) & $-1.865$ & $0.964$ \\
 & & ($49.4$,$6.2$,$81.1$) & ($18.3$,$36.8$,$7.3$) & $0.004$ & $0.034$ \\
$DTG-136$ & $6$ & ($-171.8$,$12.6$,$-87.7$) & ($760.5$,$79.4$,$150.2$) & $-1.674$ & $0.956$ \\
 & & ($20.5$,$7.2$,$34.3$) & ($15.6$,$54.0$,$8.4$) & $0.005$ & $0.015$ \\
$DTG-137$ & $6$ & ($-34.5$,$65.3$,$14.1$) & ($350.9$,$463.5$,$204.7$) & $-1.757$ & $0.700$ \\
 & & ($77.1$,$10.4$,$95.9$) & ($23.7$,$33.8$,$7.4$) & $0.016$ & $0.015$ \\
$DTG-138$ & $6$ & ($51.7$,$-91.2$,$4.6$) & ($316.0$,$-699.1$,$33.5$) & $-1.787$ & $0.618$ \\
 & & ($57.6$,$10.2$,$37.6$) & ($46.8$,$52.1$,$5.1$) & $0.012$ & $0.042$ \\
$DTG-139$ & $6$ & ($-1.7$,$154.0$,$-133.5$) & ($16.7$,$1042.6$,$373.9$) & $-1.665$ & $0.139$ \\
 & & ($24.4$,$9.7$,$49.7$) & ($9.9$,$38.2$,$18.7$) & $0.008$ & $0.039$ \\
$DTG-140$ & $6$ & ($3.9$,$224.5$,$-15.3$) & ($118.7$,$1720.2$,$196.5$) & $-1.495$ & $0.287$ \\
 & & ($104.2$,$25.6$,$86.5$) & ($31.8$,$48.2$,$9.5$) & $0.010$ & $0.041$ \\
$DTG-141$ & $6$ & ($45.2$,$2.7$,$-71.4$) & ($345.6$,$10.8$,$280.4$) & $-1.865$ & $0.863$ \\
 & & ($70.0$,$23.3$,$122.7$) & ($24.3$,$118.2$,$12.7$) & $0.017$ & $0.050$ \\
$DTG-142$ & $6$ & ($-251.3$,$-1.4$,$36.9$) & ($1228.0$,$-7.1$,$133.2$) & $-1.483$ & $0.978$ \\
 & & ($53.9$,$9.6$,$84.1$) & ($21.0$,$72.2$,$8.9$) & $0.001$ & $0.007$ \\
$DTG-143$ & $6$ & ($-106.1$,$262.1$,$-38.1$) & ($245.1$,$1810.5$,$147.3$) & $-1.447$ & $0.394$ \\
 & & ($30.9$,$28.2$,$93.0$) & ($28.1$,$53.5$,$10.6$) & $0.014$ & $0.021$ \\
$DTG-144$ & $6$ & ($-5.3$,$228.3$,$13.0$) & ($1.4$,$1892.8$,$5.1$) & $-1.563$ & $0.032$ \\
 & & ($8.1$,$1.9$,$12.4$) & ($0.6$,$11.1$,$0.8$) & $0.004$ & $0.007$ \\
$DTG-145$ & $6$ & ($-13.8$,$248.8$,$0.2$) & ($13.5$,$2033.4$,$1.7$) & $-1.521$ & $0.097$ \\
 & & ($15.3$,$13.6$,$8.5$) & ($2.9$,$1.8$,$0.5$) & $0.001$ & $0.009$ \\
$DTG-146$ & $6$ & ($-3.8$,$0.3$,$105.1$) & ($453.4$,$0.3$,$375.9$) & $-1.780$ & $0.907$ \\
 & & ($70.2$,$11.0$,$74.0$) & ($28.0$,$76.1$,$7.8$) & $0.019$ & $0.037$ \\
$DTG-147$ & $6$ & ($9.7$,$219.6$,$0.5$) & ($6.3$,$1776.6$,$4.6$) & $-1.595$ & $0.070$ \\
 & & ($13.7$,$4.3$,$15.5$) & ($1.4$,$0.6$,$0.8$) & $0.001$ & $0.008$ \\
$DTG-148$ & $6$ & ($22.4$,$210.9$,$1.5$) & ($18.8$,$1738.9$,$1.3$) & $-1.601$ & $0.122$ \\
 & & ($10.6$,$2.6$,$8.9$) & ($2.8$,$3.4$,$0.4$) & $0.002$ & $0.009$ \\
$DTG-149$ & $6$ & ($-2.3$,$253.8$,$-1.2$) & ($16.6$,$2082.7$,$2.2$) & $-1.507$ & $0.106$ \\
 & & ($18.6$,$1.7$,$10.6$) & ($2.4$,$4.3$,$0.4$) & $0.001$ & $0.008$ \\
$DTG-150$ & $6$ & ($-18.1$,$259.7$,$6.0$) & ($26.4$,$2075.0$,$1.8$) & $-1.506$ & $0.134$ \\
 & & ($21.0$,$1.7$,$5.0$) & ($2.6$,$11.5$,$0.4$) & $0.002$ & $0.007$ \\
$DTG-151$ & $6$ & ($41.4$,$238.9$,$5.0$) & ($27.6$,$1939.5$,$2.4$) & $-1.541$ & $0.141$ \\
 & & ($8.9$,$11.2$,$5.7$) & ($2.6$,$15.1$,$0.7$) & $0.003$ & $0.007$ \\
$DTG-152$ & $6$ & ($32.6$,$198.5$,$3.0$) & ($40.1$,$1655.0$,$3.3$) & $-1.619$ & $0.181$ \\
 & & ($6.5$,$3.7$,$14.0$) & ($1.9$,$5.0$,$0.7$) & $0.001$ & $0.004$ \\
\pagebreak
$DTG-153$ & $6$ & ($-1.3$,$245.6$,$-32.1$) & ($17.9$,$2008.7$,$10.0$) & $-1.522$ & $0.112$ \\
 & & ($32.1$,$5.2$,$3.3$) & ($2.9$,$4.5$,$0.9$) & $0.001$ & $0.009$ \\
$DTG-154$ & $6$ & ($1.4$,$250.3$,$-7.8$) & ($35.7$,$2020.2$,$9.3$) & $-1.514$ & $0.157$ \\
 & & ($44.3$,$8.9$,$18.8$) & ($0.7$,$13.4$,$1.1$) & $0.003$ & $0.001$ \\
$DTG-155$ & $6$ & ($-2.8$,$206.2$,$-0.3$) & ($24.5$,$1510.4$,$14.8$) & $-1.664$ & $0.148$ \\
 & & ($36.1$,$12.2$,$20.3$) & ($3.8$,$8.1$,$0.6$) & $0.002$ & $0.011$ \\
$DTG-156$ & $6$ & ($-1.4$,$37.5$,$99.9$) & ($955.7$,$297.9$,$345.4$) & $-1.476$ & $0.891$ \\
 & & ($225.2$,$13.4$,$137.2$) & ($22.1$,$93.8$,$11.7$) & $0.016$ & $0.029$ \\
$DTG-157$ & $6$ & ($9.1$,$275.5$,$11.3$) & ($65.0$,$2299.4$,$2.4$) & $-1.439$ & $0.198$ \\
 & & ($23.8$,$3.9$,$8.2$) & ($3.4$,$7.2$,$1.5$) & $0.001$ & $0.005$ \\
$DTG-158$ & $6$ & ($2.0$,$203.4$,$3.0$) & ($22.8$,$1659.0$,$24.4$) & $-1.612$ & $0.137$ \\
 & & ($27.2$,$5.7$,$29.7$) & ($6.8$,$18.6$,$1.7$) & $0.003$ & $0.020$ \\
$DTG-159$ & $6$ & ($-30.6$,$182.8$,$-9.3$) & ($109.2$,$1555.6$,$11.1$) & $-1.614$ & $0.298$ \\
 & & ($63.7$,$17.2$,$23.3$) & ($3.9$,$25.3$,$1.1$) & $0.006$ & $0.007$ \\
$DTG-160$ & $6$ & ($-11.0$,$162.9$,$27.9$) & ($62.0$,$1141.7$,$82.0$) & $-1.738$ & $0.267$ \\
 & & ($31.4$,$9.9$,$57.2$) & ($5.4$,$30.1$,$3.9$) & $0.008$ & $0.012$ \\
$DTG-161$ & $6$ & ($-52.5$,$258.0$,$14.4$) & ($71.9$,$1890.5$,$60.2$) & $-1.512$ & $0.240$ \\
 & & ($25.2$,$24.6$,$37.6$) & ($5.9$,$24.0$,$3.4$) & $0.007$ & $0.009$ \\
$DTG-162$ & $5$ & ($-31.4$,$130.8$,$-17.2$) & ($136.8$,$948.1$,$85.0$) & $-1.761$ & $0.413$ \\
 & & ($34.0$,$12.4$,$51.3$) & ($4.1$,$24.2$,$12.2$) & $0.009$ & $0.033$ \\
$DTG-163$ & $5$ & ($-32.9$,$164.7$,$42.2$) & ($45.6$,$924.1$,$73.7$) & $-1.841$ & $0.256$ \\
 & & ($23.7$,$4.5$,$54.9$) & ($7.3$,$15.5$,$5.7$) & $0.011$ & $0.018$ \\
$DTG-164$ & $5$ & ($30.5$,$69.6$,$-17.6$) & ($407.3$,$554.6$,$23.3$) & $-1.795$ & $0.712$ \\
 & & ($48.0$,$2.2$,$22.1$) & ($10.6$,$36.2$,$7.1$) & $0.015$ & $0.010$ \\
$DTG-165$ & $5$ & ($80.2$,$163.6$,$-6.9$) & ($149.9$,$1418.9$,$118.6$) & $-1.586$ & $0.354$ \\
 & & ($134.7$,$3.1$,$76.8$) & ($11.2$,$23.8$,$6.6$) & $0.008$ & $0.013$ \\
$DTG-166$ & $5$ & ($-65.8$,$42.0$,$-9.0$) & ($572.6$,$292.3$,$61.1$) & $-1.766$ & $0.847$ \\
 & & ($130.8$,$9.0$,$48.5$) & ($25.9$,$24.5$,$7.8$) & $0.008$ & $0.022$ \\
$DTG-167$ & $5$ & ($-125.1$,$-30.3$,$79.2$) & ($946.7$,$-195.8$,$437.3$) & $-1.472$ & $0.915$ \\
 & & ($276.1$,$18.9$,$173.3$) & ($35.4$,$49.4$,$18.7$) & $0.012$ & $0.018$ \\
$DTG-168$ & $5$ & ($81.4$,$8.2$,$-18.4$) & ($720.0$,$73.9$,$69.6$) & $-1.744$ & $0.948$ \\
 & & ($142.9$,$6.6$,$38.4$) & ($19.6$,$43.4$,$7.0$) & $0.015$ & $0.030$ \\
$DTG-169$ & $5$ & ($218.8$,$23.5$,$-44.9$) & ($1163.5$,$213.9$,$55.3$) & $-1.507$ & $0.920$ \\
 & & ($26.9$,$10.7$,$8.5$) & ($22.5$,$93.6$,$5.5$) & $0.022$ & $0.015$ \\
$DTG-170$ & $5$ & ($-8.1$,$-159.5$,$-19.8$) & ($145.0$,$-1264.2$,$23.0$) & $-1.699$ & $0.353$ \\
 & & ($70.9$,$14.5$,$31.5$) & ($57.2$,$6.9$,$4.1$) & $0.029$ & $0.072$ \\
$DTG-171$ & $5$ & ($4.1$,$227.0$,$-2.1$) & ($1.9$,$1843.6$,$0.3$) & $-1.580$ & $0.038$ \\
 & & ($8.1$,$3.3$,$3.3$) & ($1.0$,$2.8$,$0.5$) & $0.001$ & $0.010$ \\
\pagebreak
$DTG-172$ & $5$ & ($30.6$,$238.3$,$-17.9$) & ($15.7$,$1888.7$,$5.7$) & $-1.557$ & $0.108$ \\
 & & ($4.9$,$12.6$,$10.9$) & ($2.0$,$4.4$,$0.1$) & $0.002$ & $0.007$ \\
$DTG-173$ & $5$ & ($-41.3$,$206.3$,$2.3$) & ($31.0$,$1712.7$,$6.0$) & $-1.602$ & $0.157$ \\
 & & ($7.2$,$12.3$,$14.4$) & ($3.1$,$5.6$,$0.6$) & $0.001$ & $0.008$ \\
$DTG-174$ & $5$ & ($12.2$,$232.8$,$-31.3$) & ($8.9$,$1865.6$,$15.2$) & $-1.563$ & $0.083$ \\
 & & ($22.9$,$12.6$,$20.6$) & ($2.4$,$9.3$,$1.1$) & $0.003$ & $0.010$ \\
$DTG-175$ & $5$ & ($18.9$,$203.3$,$15.1$) & ($23.8$,$1647.9$,$13.0$) & $-1.622$ & $0.140$ \\
 & & ($28.5$,$6.0$,$25.6$) & ($2.5$,$15.3$,$0.4$) & $0.003$ & $0.008$ \\
$DTG-176$ & $5$ & ($7.5$,$154.5$,$3.6$) & ($124.0$,$1262.3$,$4.9$) & $-1.710$ & $0.345$ \\
 & & ($28.9$,$2.7$,$17.1$) & ($8.7$,$12.8$,$2.0$) & $0.003$ & $0.011$ \\
$DTG-177$ & $5$ & ($10.8$,$219.7$,$-22.0$) & ($8.7$,$1723.4$,$34.3$) & $-1.595$ & $0.088$ \\
 & & ($19.1$,$7.1$,$40.4$) & ($4.0$,$26.4$,$3.2$) & $0.008$ & $0.017$ \\
$DTG-178$ & $5$ & ($-15.9$,$157.2$,$0.4$) & ($102.2$,$1182.6$,$23.0$) & $-1.733$ & $0.324$ \\
 & & ($58.8$,$5.5$,$28.5$) & ($9.8$,$14.8$,$1.4$) & $0.000$ & $0.015$ \\
$DTG-179$ & $5$ & ($15.5$,$209.8$,$59.3$) & ($15.6$,$1515.5$,$88.1$) & $-1.630$ & $0.121$ \\
 & & ($16.5$,$24.1$,$11.4$) & ($8.2$,$12.2$,$1.8$) & $0.002$ & $0.037$ \\
\enddata
\end{deluxetable*}


==> Tables/cluster_summary_table.tex <==
\begin{deluxetable*}{l  r  r  c}
\tabletypesize{\scriptsize}
\tablecaption{Identified DTGs \label{tab:cluster_summary}}
\tablehead{\colhead{DTG} & \colhead{$N$ Stars} & \colhead{Confidence} & \colhead{Associations}}
\startdata
1 & $35$ & $99.0\%$ & new\\
2 & $30$ & $79.0\%$ & DS21:DTG-13\\
3 & $30$ & $93.0\%$ & new\\
4 & $28$ & $90.5\%$ & DS21:DTG-4, DG21:CDTG-18, GM18a:C1, HL19:GL-2, GL21:DTG-8\\
5 & $27$ & $77.1\%$ & Splashed Disk\\
6 & $24$ & $59.1\%$ & DS21:DTG-47\\
7 & $23$ & $87.7\%$ & GSE, IR18:E, DG21:CDTG-1, EV21:NGC~4833, GC21:Sausage, GL21:DTG-37, DS21:DTG-43\\
8 & $23$ & $95.5\%$ & GSE, DS21:DTG-3, GC21:Sausage, DG21:CDTG-9, GL21:DTG-34\\
9 & $23$ & $86.4\%$ & new\\
10 & $22$ & $98.9\%$ & DS21:DTG-12\\
11 & $22$ & $90.5\%$ & new\\
12 & $21$ & $58.9\%$ & GSE, GM17:Comoving, EV21:Ryu~879~(RLGC~2)\\
13 & $21$ & $74.1\%$ & new\\
14 & $20$ & $59.3\%$ & MWTD, DG21:CDTG-6, HL19:GL-1, DS21:DTG-2\\
15 & $20$ & $91.8\%$ & Splashed Disk, DG21:CDTG-5\\
16 & $20$ & $61.4\%$ & new\\
17 & $19$ & $67.3\%$ & GSE, DS21:DTG-17, GC21:Sausage, GL21:DTG-37\\
18 & $19$ & $60.0\%$ & GSE, EV21:NGC~5139~($\omega$Cen)\\
19 & $19$ & $66.3\%$ & DS21:DTG-23\\
20 & $18$ & $73.4\%$ & GSE, HL20:GR-1, DG21:CDTG-19, DS21:DTG-29\\
21 & $18$ & $99.3\%$ & new\\
22 & $17$ & $84.5\%$ & MWTD\\
23 & $17$ & $62.1\%$ & new\\
24 & $16$ & $63.8\%$ & GSE, GC21:Sausage\\
25 & $15$ & $91.0\%$ & DG21:CDTG-23\\
26 & $15$ & $64.8\%$ & GSE, AH17:VelHel-6, DS21:DTG-5\\
27 & $15$ & $68.9\%$ & GSE, HL20:GR-1, DS21:DTG-17\\
28 & $15$ & $72.1\%$ & GSE, SM20:Sausage, GC21:Sausage, DS21:DTG-27\\
29 & $14$ & $97.7\%$ & MWTD, AH17:VelHel-6\\
30 & $14$ & $54.7\%$ & GSE, AH17:VelHel-5, DG21:CDTG-28, GC21:Sausage\\
31 & $14$ & $81.2\%$ & DS21:DTG-30\\
32 & $14$ & $76.4\%$ & new\\
33 & $13$ & $98.5\%$ & EV21:NGC~6752\\
34 & $13$ & $60.6\%$ & new\\
35 & $13$ & $95.5\%$ & new\\
36 & $13$ & $81.4\%$ & new\\
37 & $12$ & $69.0\%$ & MWTD\\
38 & $12$ & $70.7\%$ & HL19:GL-1\\
39 & $12$ & $99.4\%$ & new\\
40 & $12$ & $70.7\%$ & new\\
41 & $12$ & $83.3\%$ & new\\
42 & $12$ & $82.5\%$ & Helmi Stream, HK18:Green, NB20:H99, GM18a:S2, GM18b:S2, DG21:CDTG-15, GL21:DTG-3\\
43 & $11$ & $75.7\%$ & MWTD\\
44 & $11$ & $97.9\%$ & GSE, AH17:VelHel-6\\
45 & $11$ & $61.9\%$ & GSE, GC21:Sausage\\
46 & $11$ & $64.8\%$ & GSE, DG21:CDTG-13, AH17:VelHel-5\\
47 & $11$ & $81.4\%$ & Thamnos, AH17:VelHel-4, GC21:Sequoia\\
48 & $11$ & $72.2\%$ & new\\
49 & $11$ & $60.0\%$ & new\\
50 & $11$ & $57.1\%$ & GSE, NB20:Enc, SM20:Sausage, GC21:Sausage\\
51 & $11$ & $92.3\%$ & DG21:CDTG-3\\
52 & $10$ & $78.0\%$ & Thamnos, GC21:Sequoia, EV21:NGC~6356\\
53 & $10$ & $54.1\%$ & DS21:DTG-2\\
54 & $10$ & $98.6\%$ & new\\
55 & $10$ & $99.8\%$ & EV21:NGC~6397, DS21:DTG-9\\
56 & $10$ & $68.1\%$ & GSE\\
57 & $10$ & $54.6\%$ & GSE, GC21:Sausage, DS21:DTG-11, EV21:Ryu~879~(RLGC~2)\\
58 & $10$ & $60.1\%$ & GSE, GM17:Comoving, GC21:Sausage, EV21:Ryu~879~(RLGC~2)\\
59 & $10$ & $72.5\%$ & new\\
60 & $10$ & $78.6\%$ & new\\
61 & $10$ & $62.9\%$ & new\\
62 & $10$ & $76.4\%$ & new\\
63 & $10$ & $62.3\%$ & new\\
64 & $10$ & $96.6\%$ & new\\
65 & $10$ & $88.7\%$ & MWTD\\
66 & $10$ & $62.1\%$ & GSE, SM20:Sausage, GC21:Sausage, EV21:IC~1257\\
67 & $10$ & $95.4\%$ & LMS-1, DG21:CDTG-4, GM17:Comoving, GM18a:C1, GM18b:Cand11, GL21:DTG-2\\
68 & $9$ & $95.1\%$ & new\\
69 & $9$ & $70.5\%$ & GSE, AH17:VelHel-6\\
70 & $9$ & $92.6\%$ & GSE, AH17:VelHel-6, DG21:CDTG-22\\
71 & $9$ & $96.5\%$ & GSE, AH17:VelHel-6, GL21:DTG-37\\
72 & $9$ & $86.1\%$ & new\\
73 & $9$ & $68.5\%$ & new\\
74 & $9$ & $62.1\%$ & new\\
75 & $9$ & $50.9\%$ & GSE, DS21:DTG-8, GM17:Comoving, SM20:Sausage, GC21:Sausage\\
76 & $9$ & $78.8\%$ & GSE\\
77 & $9$ & $86.3\%$ & new\\
78 & $9$ & $58.6\%$ & GSE, DG21:CDTG-14\\
79 & $9$ & $58.7\%$ & GSE, GM17:Comoving, GC21:Sausage, DG21:CDTG-7\\
80 & $9$ & $53.6\%$ & GSE, GM17:Comoving, GC21:Sausage\\
81 & $9$ & $62.3\%$ & new\\
82 & $9$ & $73.3\%$ & new\\
83 & $9$ & $81.3\%$ & new\\
84 & $9$ & $70.5\%$ & new\\
85 & $9$ & $72.3\%$ & new\\
86 & $9$ & $65.8\%$ & Splashed Disk\\
87 & $9$ & $100.0\%$ & new\\
88 & $9$ & $91.3\%$ & new\\
89 & $9$ & $61.5\%$ & new\\
90 & $8$ & $73.5\%$ & MWTD, DS21:DTG-44\\
91 & $8$ & $52.1\%$ & new\\
92 & $8$ & $52.1\%$ & GSE, SM20:Sausage, GC21:Sausage, GL21:DTG-11, DS21:DTG-42\\
93 & $8$ & $84.0\%$ & AH17:VelHel-6\\
94 & $8$ & $99.5\%$ & AH17:VelHel-7\\
95 & $8$ & $95.9\%$ & GSE, DS21:DTG-36\\
96 & $8$ & $84.5\%$ & GSE\\
97 & $8$ & $56.9\%$ & GSE, HL20:GR-1\\
98 & $8$ & $79.8\%$ & GSE, AH17:VelHel-1, AH17:VelHel-2, GC21:Sausage\\
99 & $8$ & $53.5\%$ & HL19:GL-1\\
100 & $8$ & $64.1\%$ & GSE\\
101 & $8$ & $64.0\%$ & new\\
102 & $8$ & $87.6\%$ & Thamnos, HL20:GR-2, DG21:CDTG-2\\
103 & $8$ & $71.5\%$ & DS21:DTG-19\\
104 & $8$ & $87.6\%$ & new\\
105 & $8$ & $74.0\%$ & new\\
106 & $7$ & $60.6\%$ & MWTD\\
107 & $7$ & $56.0\%$ & MWTD\\
108 & $7$ & $68.0\%$ & new\\
109 & $7$ & $73.6\%$ & new\\
110 & $7$ & $49.7\%$ & MWTD\\
111 & $7$ & $69.3\%$ & GSE, DG21:CDTG-12\\
112 & $7$ & $68.4\%$ & GSE\\
113 & $7$ & $72.8\%$ & GSE\\
114 & $7$ & $50.1\%$ & GSE, HL20:GR-1\\
115 & $7$ & $50.9\%$ & GSE, GC21:Sausage\\
116 & $7$ & $53.6\%$ & GSE\\
117 & $7$ & $47.9\%$ & new\\
118 & $7$ & $53.2\%$ & new\\
119 & $7$ & $53.3\%$ & DS21:DTG-1\\
120 & $7$ & $45.5\%$ & new\\
121 & $7$ & $98.7\%$ & new\\
122 & $7$ & $71.6\%$ & new\\
123 & $7$ & $93.2\%$ & new\\
124 & $7$ & $66.3\%$ & AH17:VelHel-7, DG21:CDTG-23\\
125 & $7$ & $88.9\%$ & new\\
126 & $7$ & $82.0\%$ & new\\
127 & $7$ & $62.4\%$ & GC21:Sequoia\\
128 & $7$ & $83.8\%$ & new\\
129 & $7$ & $51.0\%$ & new\\
130 & $6$ & $73.0\%$ & new\\
131 & $6$ & $55.1\%$ & new\\
132 & $6$ & $50.0\%$ & MWTD, AH17:VelHel-7\\
133 & $6$ & $82.4\%$ & GSE, AH17:VelHel-6, DS21:DTG-22\\
134 & $6$ & $29.1\%$ & GSE, GC21:Sausage\\
135 & $6$ & $48.5\%$ & GSE, GC21:Sausage, DS21:DTG-29\\
136 & $6$ & $23.9\%$ & GSE, GC21:Sausage\\
137 & $6$ & $64.9\%$ & GSE\\
138 & $6$ & $64.5\%$ & Thamnos, HL20:GR-2, GC21:Sequoia\\
139 & $6$ & $39.1\%$ & new\\
140 & $6$ & $66.4\%$ & new\\
141 & $6$ & $43.4\%$ & GSE, HL20:GR-1, DG21:CDTG-7, EV21:NGC~6284\\
142 & $6$ & $76.5\%$ & GSE, GC21:Sausage\\
143 & $6$ & $78.9\%$ & new\\
144 & $6$ & $29.0\%$ & new\\
145 & $6$ & $66.2\%$ & new\\
146 & $6$ & $67.4\%$ & GSE, GC21:Sausage\\
147 & $6$ & $51.9\%$ & DS21:DTG-1\\
148 & $6$ & $38.9\%$ & DS21:DTG-1\\
149 & $6$ & $25.8\%$ & new\\
150 & $6$ & $38.3\%$ & new\\
151 & $6$ & $46.2\%$ & new\\
152 & $6$ & $72.2\%$ & new\\
153 & $6$ & $67.0\%$ & new\\
154 & $6$ & $62.4\%$ & new\\
155 & $6$ & $63.6\%$ & new\\
156 & $6$ & $66.2\%$ & GSE, AH17:VelHel-2\\
157 & $6$ & $99.7\%$ & new\\
158 & $6$ & $89.2\%$ & new\\
159 & $6$ & $97.3\%$ & new\\
160 & $6$ & $62.6\%$ & new\\
161 & $6$ & $94.3\%$ & new\\
162 & $5$ & $69.9\%$ & new\\
163 & $5$ & $56.8\%$ & DS21:DTG-14\\
164 & $5$ & $64.2\%$ & GSE, DG21:CDTG-22\\
165 & $5$ & $51.7\%$ & new\\
166 & $5$ & $45.5\%$ & GSE, AH17:VelHel-6\\
167 & $5$ & $51.0\%$ & GSE\\
168 & $5$ & $80.4\%$ & GSE, GC21:Sausage\\
169 & $5$ & $57.7\%$ & GSE\\
170 & $5$ & $69.0\%$ & Thamnos, SM20:SeqG1, GL21:DTG-25\\
171 & $5$ & $54.0\%$ & new\\
172 & $5$ & $29.0\%$ & new\\
173 & $5$ & $66.2\%$ & new\\
174 & $5$ & $97.8\%$ & new\\
175 & $5$ & $60.1\%$ & new\\
176 & $5$ & $53.3\%$ & DG21:CDTG-5\\
177 & $5$ & $64.6\%$ & new\\
178 & $5$ & $92.8\%$ & new\\
179 & $5$ & $77.4\%$ & new\\
\enddata
\tablecomments{We adopt the nomenclature for previously identified DTGs and CDTGs from \cite{Yuan2020b}.}\end{deluxetable*}


==> Tables/full_data_description_table.tex <==
\startlongtable
\begin{deluxetable*}{c  l  l  l}
\tablecaption{Description of the Full Sample from the RAVE Survey \label{tab:full_data_descript}}
\tablehead{\colhead{Column} & \colhead{Field} & \colhead{Unit} & \colhead{Description}}
\startdata
1 & RAVE ID & $-$ & The RAVE DR6 RAVE ID of the star\\
2 & Source ID & $-$ & The Gaia EDR3 Source ID of the star\\
3 & SMSS ID & $-$ & The SMSS DR2 Source ID of the star\\
4 & RAVE NAME & $-$ & The RAVE DR6 RAVE NAME of the star\\
5 & RA & (J2000) & The Right Ascension of the star given in hours:minutes:seconds\\
6 & DEC & (J2000) & The Declination of the star given in degrees:minutes:seconds\\
7 & Telescope & $-$ & The telescope that was used to obtain the spectrum of the star\\
8 & $V_{\rm mag}$ & $-$ & The $V$ magnitude of the star as given by the $V_{\rm mag}$ Reference\\
9 & $G_{\rm mag}$ & $-$ & The Gaia $G$ mean magnitude of the star as given by the Gaia Source ID\\
10 & $G_{\rm BP} - G_{\rm RP}$ & $-$ & The Gaia BP $-$ RP color mean magnitude of the star as given by the Gaia Source ID\\
11 & $V_{\rm mag}$ (Gaia) & $-$ & The $V$ magnitude of the star as determined by the transformations from G mag to V mag using\\
 &  &  & $V$ $=$ $G$ $+$ $0.02704$ $-$ $0.01424*(\rm{BP}-\rm{RP})$ $+$ $0.2156*(\rm{BP}-\rm{RP})^2$ $-$\\
 &  &  & $0.01426(\rm{BP}-\rm{RP})^3$ given by \citet{Riello2021}\\
12 & RV$_{\rm RAVE}$ & (km s$^{-1}$) & The radial velocity as given by the RAVE ID\\
13 & Error & (km s$^{-1}$) & The radial velocity error as given by the RAVE ID\\
14 & RV$_{\rm Gaia}$ & (km s$^{-1}$) & The radial velocity as given by the Gaia Source ID\\
15 & Error & (km s$^{-1}$) & The radial velocity error as given by the Gaia Source ID\\
16 & Parallax & (mas) & The parallax as given by the Gaia Source ID\\
17 & Error & (mas) & The parallax error as given by the Gaia Source ID\\
18 & Distance & (kpc) & The inverse parallax distance (1/Parallax)\\
19 & Error & (kpc) & The inverse parallax distance error (Parallax$_{error}$/(Parallax$^2$))\\
20 & Distance$_{\rm Corrected}$ & (kpc) & The corrected inverse parallax distance (1/(Parallax + 0.026)) based on \citet{Huang2021a}\\
21 & Error & (kpc) & The corrected inverse parallax distance error (Parallax$_{error}$/((Parallax + 0.026)$^2$))\\
 &  &  & based on \citet{Huang2021a}\\
22 & Relative Error & $-$ & The relative error of the corrected distance as given by Gaia\\
23 & Distance BJ21 & (kpc) & The 50 percentile distance as given by \citet{Bailer-Jones2021} based on the Gaia Source ID\\
24 & Error & (kpc) & The 50 percentile error as estimated by the 84 percentile distance and the 16 percentile\\
 &  &  & distance as given by \citet{Bailer-Jones2021} based on the Gaia Source ID ((dist84-dist16)/2)\\
25 & Relative Error & $-$ & The relative error of the 50 percentile distance as given by \citet{Bailer-Jones2021} based on\\
 &  &  & the Gaia Source ID\\
26 & Distance StarHorse & (kpc) & The 50 percentile distance as given by \citet{Anders2021} based on the Gaia Source ID\\
27 & Error & (kpc) & The 50 percentile error as estimated by the 84 percentile distance and the 16 percentile\\
 &  &  & distance as given by \citet{Anders2021} based on the Gaia Source ID ((dist84-dist16)/2)\\
28 & Relative Error & $-$ & The relative error of the 50 percentile distance as given by \citet{Anders2021} based on the\\
 &  &  & Gaia Source ID\\
29 & PM$_{\rm RA}$ & (mas yr$^{-1}$) & The proper motion in the Right Ascension as given by the Gaia Source ID\\
30 & Error & (mas yr$^{-1}$) & The proper motion error in the Right Ascension as given by the Gaia Source ID\\
31 & PM$_{\rm DEC}$ & (mas yr$^{-1}$) & The proper motion in the Declination as given by the Gaia Source ID\\
32 & Error & (mas yr$^{-1}$) & The proper motion error in the Declination as given by the Gaia Source ID\\
33 & Correlation Coefficient & $-$ & The correlation coefficient between the proper motion in Right Ascension and the proper motion\\
 &  &  & in Declination as given by the Gaia Source ID\\
34 & T$_{\rm eff~RAVE}$ & (K) & The effective temperature of the star as given by the RAVE ID\\
35 & Error & (K) & The effective temperature error of the star as given by the RAVE ID\\
36 & T$_{\rm eff~Spec}$ & (K) & The effective temperature of the star as given by the n-SSPP\\
37 & Error & (K) & The effective temperature error of the star as given by the n-SSPP\\
38 & T$_{\rm eff~Phot}$ & (K) & The effective temperature of the star as given by \citet{Huang2021c}\\
39 & Error & (K) & The effective temperature error of the star as given by \citet{Huang2021c}\\
40 & T$_{\rm eff}$ & (K) & The adopted effective temperature of the star based on the Parameter Procedure\\
41 & Error & (K) & The adopted effective temperature error of the star based on the Parameter Procedure\\
42 & log \textit{g}$_{\rm RAVE}$ & (cgs) & The surface gravity of the star as given by the RAVE ID\\
43 & Error & (cgs) & The surface gravity error of the star as given by the RAVE ID\\
44 & log \textit{g}$_{\rm Spec}$ & (cgs) & The surface gravity of the star as given by the n-SSPP\\
\pagebreak \\[-3.5ex]
45 & Error & (cgs) & The surface gravity error of the star as given by the n-SSPP\\
46 & log \textit{g} & (cgs) & The adopted surface gravity of the star based on the Parameter Procedure\\
47 & Error & (cgs) & The adopted surface gravity error of the star based on the Parameter Procedure\\
48 & [M/H] & $-$ & The metallicity of the star as given by the RAVE ID\\
49 & Error & $-$ & The metallicity error of the star as given by the RAVE ID\\
50 & [Fe/H]$_{Spec}$ & $-$ & The metallicity of the star as given by the n-SSPP\\
51 & Error & $-$ & The metallicity error of the star as given by the n-SSPP\\
52 & [Fe/H]$_{Phot}$ & $-$ & The metallicity of the star as given by \citet{Huang2021c}\\
53 & Error & $-$ & The metallicity error of the star as given by \citet{Huang2021c}\\
54 & [Fe/H] & $-$ & The adopted metallicity of the star based on the Parameter Procedure\\
55 & Error & $-$ & The adopted metallicity error of the star based on the Parameter Procedure\\
56 & [C/Fe] & $-$ & The carbon abundance ratio for the star\\
57 & Error & $-$ & The carbon abundance ratio error for the star\\
58 & [C/Fe]$_{c}$ & $-$ & The carbon abundance corrected for evolutionary effects from \citet{Placco2014}\\
59 & AC$_{c}$ & $-$ & The absolute carbon corrected for evolutionary effects from \citet{Placco2014} ([C/Fe]$_{c}$ +\\
 &  &  & [Fe/H] + log($\epsilon$)$_{Carbon,Solar}$) (Taken from solar value of 8.43 from\\
 &  &  & \citet{Asplund2009})\\
60 & CARDET & $-$ & Flag with ``D" if the carbon abundance ([C/Fe]) is detected from n-SSPP and ``U" if an upper\\
 &  &  & limit by n-SSPP and ``L" if a lower limit by n-SSPP and ``N" if none is detected by n-SSPP\\
61 & CC$_{\rm [C/Fe]}$ & $-$ & The correlation coefficient of [C/Fe] as given by the n-SSPP\\
62 & CEMP & $-$ & Flag as ``C" for Carbon-Enhanced Metal-Poor (CEMP) if [C/Fe]$_{c}$ $> +0.7$ and ``I" for\\
 &  &  & CEMP-intermediate if $+0.5 <$ [C/Fe]$_{c}$ $\leq +0.7$ and ``N" for Carbon-Normal if\\
 &  &  & [C/Fe]$_{c}$ $\leq +0.5$ and ``X" if there is no [C/Fe]$_{c}$ information\\
63 & [$\alpha$/Fe]$_{\rm RAVE}$ & $-$ & The alpha-element abundance ratio for the star as given by the RAVE ID\\
64 & Error & $-$ & The alpha-element abundance ratio error for the star as given by the RAVE ID\\
65 & [$\alpha$/Fe]$_{\rm Spec}$ & $-$ & The alpha-element abundance ratio for the star as given by the n-SSPP\\
66 & Error & $-$ & The alpha-element abundance ratio error for the star as given by the n-SSPP\\
67 & ALPDET & $-$ & Flag with ``D" if the alpha abundance ([$\alpha$/Fe]) is detected from n-SSPP and ``U" if an\\
 &  &  & upper limit by n-SSPP and ``L" if a lower limit by n-SSPP and ``N" if none is detected by\\
 &  &  & n-SSPP\\
68 & CC$_{\rm{[}\alpha\rm{/Fe]}}$ & $-$ & The correlation coefficient of [$\alpha$/Fe] as detected by the n-SSPP\\
69 & [$\alpha$/Fe] & $-$ & The alpha-element abundance ratio for the star based on the Parameter Procedure\\
70 & Error & $-$ & The alpha-element abundance ratio error for the star based on the Parameter Procedure\\
71 & SNR & $-$ & The average Signal-to-Noise Ratio of the spectrum from the RAVE ID\\
72 & Reference & $-$ & The Reference for the star as given by ``RAVE DR6" for the sample of stars from\\
 &  &  & \citet{Steinmetz2020a} sample and ``RAVE DR5" for the sample of stars from \citet{Kunder2017}\\
73 & Parameter Procedure & $-$ & The procedure used to determine the adopted stellar parameters (T$_{\rm eff}$, log \textit{g},\\
 &  &  & [Fe/H], and [$\alpha$/Fe]) (``Average" is used if the difference between [Fe/H]$_{Spec}$ and\\
 &  &  & [Fe/H]$_{Phot}$ is less $\leq$\ 0.5 dex and ``Spectroscopic" is used if only [Fe/H]$_{Spec}$\\
 &  &  & is available and ``Photometric" is used if only [Fe/H]$_{Phot}$ is available, while a choice\\
 &  &  & is made between [Fe/H]$_{Spec}$ and [Fe/H]$_{Phot}$ if both are available and the difference\\
 &  &  & is $>$ 0.5 dex)\\
74 & $V_{\rm mag}$ Reference & $-$ & The Reference for the \textit{V} magnitude of the star\\
75 & Distance AGAMA & $-$ & The Reference for the distance used in AGAMA (StarHorse prioritized over BJ21 unless StarHorse\\
 &  &  & distance has relative error greater than 0.3, if both have a relative error greater than 0.3\\
 &  &  & we adopt no distance estimate)\\
76 & RV Reference & $-$ & The Reference for the RV\\
\enddata
\end{deluxetable*}

